AANet: Attribute Attention Network for Person Re-Identifications

This paper proposes Attribute Attention Network (AANet), a new architecture that integrates person attributes and attribute attention maps into a classification framework to solve the person re-identification (re-ID) problem. Many person re-ID models typically employ semantic cues such as body parts or human pose to improve the re-ID performance. Attribute information, however, is often not utilized. The proposed AANet leverages on a baseline model that uses body parts and integrates the key attribute information in an unified learning framework. The AANet consists of a global person ID task, a part detection task and a crucial attribute detection task. By estimating the class responses of individual attributes and combining them to form the attribute attention map (AAM), a very strong discriminatory representation is constructed. The proposed AANet outperforms the best state-of-the-art method arXiv:1711.09349v3 [cs.CV] using ResNet-50 by 3.36% in mAP and 3.12% in Rank-1 accuracy on DukeMTMC-reID dataset. On Market1501 dataset, AANet achieves 92.38% mAP and 95.10% Rank-1 accuracy with re-ranking, outperforming arXiv:1804.00216v1 [cs.CV], another state of the art method using ResNet-152, by 1.42% in mAP and 0.47% in Rank-1 accuracy. In addition, AANet can perform person attribute prediction (e.g., gender, hair length, clothing length etc.), and localize the attributes in the query image.

==> AANet-cvpr2019_v10.tex <==
%\documentclass[10pt,twocolumn,letterpaper]{article}

%\documentclass[10pt,letterpaper]{article}
%\usepackage{multicol}

\usepackage{cvpr}
\usepackage{times}
\usepackage{epsfig}
\usepackage{graphicx}
\usepackage{amsmath}
\usepackage{amssymb}

\usepackage{array}
\newcolumntype{L}[1]{>{\raggedright\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\newcolumntype{C}[1]{>{\centering\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\newcolumntype{R}[1]{>{\raggedleft\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}

% Include other packages here, before hyperref.

% If you comment hyperref and then uncomment it, you should delete
% egpaper.aux before re-running latex.  (Or just hit 'q' on the first latex
% run, let it finish, and you should be clear).
\usepackage[pagebackref=true,breaklinks=true,letterpaper=true,colorlinks,bookmarks=false]{hyperref}

% \cvprfinalcopy % *** Uncomment this line for the final submission

\def\cvprPaperID{****} % *** Enter the CVPR Paper ID here
\def\httilde{\mbox{\tt\raisebox{-.5ex}{\symbol{126}}}}

% Pages are numbered in submission mode, and unnumbered in camera-ready
\ifcvprfinal\pagestyle{empty}\fi
\begin{document}

%%%%%%%%% TITLE
\title{AANet: Attribute Attention Network for Person Re-Identifications}

\author{First Author\\
Institution1\\
Institution1 address\\
{\tt\small firstauthor@i1.org}
% For a paper whose authors are all at the same institution,
% omit the following lines up until the closing ``}''.
% Additional authors and addresses can be added with ``\and'',
% just like the second author.
% To save space, use either the email address or home page, not both
\and
Second Author\\
Institution2\\
First line of institution2 address\\
{\tt\small secondauthor@i2.org}
}

\maketitle
%\thispagestyle{empty}

%\begin{multicols}{2}

%%%%%%%%% ABSTRACT
\begin{abstract}
   %The ABSTRACT is to be in fully-justified italicized text, at the top
   %of the left-hand column, below the author and affiliation
   %information. Use the word ``Abstract'' as the title, in 12-point
   %Times, boldface type, centered relative to the column, initially
   %capitalized. The abstract is to be in 10-point, single-spaced type.
   %Leave two blank lines after the Abstract, then begin the main text.
   %Look at previous CVPR abstracts to get a feel for style and length.
   
   %In this paper, we propose a new person re-identification (re-ID) method by using person attributes, and by learning the merged regions indicated by class sensitive localized neuron responses from individual attributes, to assist the main identity classification task. We call this the  Attribute Attention Network (AANet). A person re-ID model usually requires additional cues, such as body parts or human pose estimation to enhance the prediction job. We built our baseline network using the same concept. Our AANet consists of the main identification task with a sub task to detect body parts. We then integrate a crucial attribute detection task, which extracts class sensitive regions for learning. We believe that there are many useful features hidden within the Convolutional Neural Network (CNN). By searching for class aware responses of the individual attributes and combining them to form the attribute attention map (AAM), we arrived at a person re-ID network that has very strong discriminatory representations. When benchmark against the work done by Sun \etal \cite{Sun_2018_ECCV}, which is the best state-of-the-art method with ResNet-50, we outperform it by 3.36\% mAP and 3.12\% Rank-1 accuracy on DukeMTMC-reID dataset. On the Market1501 dataset, we outperform the same work by 0.8\% mAP and 0.08\% Rank-1 accuracy. We also outperform other state-of-the-art methods utilizing deeper backbone architectures. Our AANet, trained with ResNet-152, achieves 92.38\% mAP and 95.10\% Rank-1 in re-rank accuracy. Furthermore, we have the ability to predict person attribute, giving our user a flexible and powerful text-based query system for person image retrieval.
   
   This paper proposes Attribute Attention Network (AANet), a new architecture that integrates person attributes and attribute attention maps into a classification framework to solve the person re-identification (re-ID) problem. Many person re-ID models typically employ semantic cues such as body parts or human pose to improve the re-ID performance. Attribute information, however, is often not utilized. The proposed AANet leverages on a baseline model that uses body parts and integrates the key attribute information in an unified learning framework. The AANet consists of a global person ID task, a part detection task and a crucial attribute detection task. By estimating the class responses of individual attributes and combining them to form the attribute attention map (AAM), a very strong discriminatory representation is constructed. The proposed AANet outperforms the best state-of-the-art method \cite{Sun_2018_ECCV} by 3.36\% in mAP and 3.12\% in Rank-1 accuracy on DukeMTMC-reID dataset. On Market1501 dataset, AANet achieves 92.38\% mAP and 95.10\% Rank-1 with re-ranking, outperforming~\cite{Sun_2018_ECCV} by 0.8\% in mAP and 0.08\% in Rank-1 accuracy. We also outperform other state-of-the-art methods utilizing deeper backbone architectures. In addition, AANet can perform person attribute prediction (e.g., gender, hair length, clothing length etc.), and localize the attributes in the query image. 
   
\end{abstract}

%%%%%%%%% BODY TEXT
\section{Introduction}

%Conventionally, person re-ID aims to retrieve images of a person taken from an array of cameras, or from same camera but from different occasions, by using a query image. Usually this prediction task is limited to a short time frame and within a small geographical area. This seemingly simple recognition task to human is a challenge to the machine, as factors like person occlusions, pose variation, ambient light changes, low image resolution, etc. degrade image quality and reduce effective number of usable pixels for image processing. In recent years, deep learning has overcome many limitations, and improves the retrieval performance significantly. Still, there are many rooms for improvement.

Given a query image, person re-ID aims to retrieve images of a queried person from a collection of images from a network of cameras. The retrieval is typically attempted from a collection of images acquired within a short time interval with respect to the queried image. This supports the underlying assumption that the query peron's appearance and clothing attributes remain unchanged across the query and the collection images. Person re-ID is a challenging problem due to many factors such as partial/total occlusion of the subject, pose variation, ambient light changes, low image resolution, etc. Recent deep learning based re-ID solutions have demonstrated good retrieval performance. 

%\par One important person re-ID application is in the camera surveillance domain. Tens of thousands of cameras are being installed in cities all over the world, and these cameras are expected to not just record videos, but also perform identification of person attribute. Some examples of useful person attribute information are gender, hair, hat, clothing colors and types and carried bags. This prediction ability, however, is lacking in most person re-ID network.

\begin{figure}
\centering
\includegraphics[width=\linewidth]{merged_attributes_id33.jpg}
\caption{Class-aware attribute attention maps are extracted and combined together to form a discriminatory feature map at the image level. The six attention maps shown in the figure correspond to the six attributes such as hair, upper clothing color, lower clothing color etc. Best viewed in color.}
\label{fig:MergedAttribute}
\end{figure}

\begin{figure*}
\centering
\includegraphics[width=\linewidth]{AANet_v3.jpg}
\caption{Overview of AANet. The backbone network is based on ResNet architecture. The backbone network outputs the feature map \(X\). The feature map \(X\) is forwarded to three tasks, namely the Global Feature Network(GFN), Part Feature Network (PFN) and Attribute Feature Network (AFN). The output of these three tasks are combined using homoscedastic uncertainty learning to predict the person identification. Best viewed in color.}
\label{fig:AANet}
\end{figure*}


%\par In this work, we aim for good person re-ID performance with person attribute prediction capability. To achieve our goals, we look to multitask network, with a person identification (ID) main task, and two relevant  attribute and body part detection sub tasks. The main task performs global feature learning. The two sub tasks, however, perform localized and different feature learning. By sharing their learning experience with the main task, we have a very discriminatory representations at the output of the network. This is shown in Figure \ref{fig:AANet}. AANet consists of two main networks. The first main network performs global identity classification, and body part detection and classification. This two tasks are managed by the Global Feature Network (GFN) and the Part Feature Network (PFN). The second main network is the Attribute Feature Network (AFN), which also consists of two tasks, namely the person attribute classification and AAM classification. All four tasks utilizes Softmax classification outputs, using image labels and person attribute labels as ground truth for learning. To ensure optimal performance, we use uncertainty learning to obtain the weighting for each task. The final task loss is then the summation of the scaled task losses.

\par The approaches used to solve the person re-ID problem can be broadly divided into two categories. The first category comprises of metric learning methods that attempt to learn an embedding space which brings images belonging to a unique person close together and those belonging to different persons far away. Various distance metrics such as triplet and quadruplet losses have been employed to learn such embedding spaces \cite{DBLP:journals/corr/HermansBL17, chen2017beyond}.

\par The second category of methods poses the re-ID problem as a identity classiﬁcation problem based on the input query image. Research has shown that by integrating semantic information such as body parts, human pose etc, the classiﬁcation and recognition accuracy can be signiﬁcantly improved \cite{DBLP:conf/iccv/SuLZX0T17, DBLP:conf/mm/WeiZY0T17, DBLP:journals/corr/YaoZZLT17}. Person attributes, such as clothing color, hair, presence/absence of backpack, etc. are, however, not used by the current state-of-the-art re-ID solutions. Since, in person re-ID it is assumed that the physical appearance of the person of interest does not significantly change between query image and the search images, the person's attributes forms a key information that can be mined to achieve higher re-ID performances. Such information is not utilized by current research and the state-of- the-art re-ID methods. 
\par In this work, we propose to integrate the person attribute information into the identity classiﬁcation framework. The resulting framework, called the Attribute Attention Network (AANet), brings together identity classiﬁcation, body part detection and person attributes into an unified framework that jointly learns a highly discriminatory feature space. The resulting network outperforms existing state-of-the-art methods in multiple benchmark datasets.  
%\par We believe that there are many discriminatory features hidden within our AANet. Object discovery with deep neural networks has been shown by Le \etal \cite{le2013building} in an unsupervised way in 2013. Zhou \etal \cite{zhou2014object} showed that for a CNN trained for scene recognition, the object detection with no supervision emerges even more than that trained with ImageNet. When the CNN is setup for scene classification with supervision, many more object can be discovered than in object classification. Inspired by this, we set out to treat our person attributes as objects and the global image as scene. We use Class-Activation Mapping (CAM) \cite{zhou2016learning} as object detector to localize the regions belonging to the person attributes. Only those attributes which exhibit strong visual cue of the human subject are combined to form a map with strong discriminatory features. This idea is shown in Figure \ref{fig:MergedAttribute}. We are not performing semantic segmentation, and thus not expecting the map to resemble fully that of the input person image. However, we can see from Figure \ref{fig:MergedAttribute} that the produced combined map gives us strong discriminatory features very useful for learning. The spatial information of the attribute objects, and their spatial relationships to each others are well captured. In addition, the background clutters are removed in most cases. This renders a more generalized network. A comparison between the AAM and global ID heat map are shown in Figure \ref{fig:AAM_Heatmap}. The AAM map follows more closely to the pedestrian shape, whereas the global ID heat map reveals whatever regions that the trained network thinks are discriminatory for ID classification, which explains why ID classification alone tends to over-fit. Thus, AAM as a relevant task in a multitask network, shares its learning experience and helps to regularize the main task.

\par Figure \ref{fig:AANet} gives an overview of the proposed architecture. The proposed framework consists of three sub-networks. The first network, called the Global Feature Network (GFN), performs global identity (ID) classiﬁcation based on the input query image. The second network, called the Part Feature Network (PFN), focuses on body part detection. The third network is the Attribute Feature Network (AFN), which extracts information from the person's attributes. The three networks perform classiﬁcation using person ID and attribute lables. We use homoscedastic uncertainty learning to optimize the weights of the three sub-tasks for the final loss calculations.

\par Since AANet performs person attribute classification as part of solving the re-id problem, AANet also produces text-based attribute descriptions for each query image along with the localized regions where the respective attributes are found in the query image. 

\par Our key contributions can be summarized as follows:
\begin{enumerate}
    \item We provide a new network architecture that integrates attribute features with identity and body part classification in a uniﬁed learning framework.

    \item We outperform the existing best state-of-the-art re-ID methods on multiple benchmark datasets and propose the new state-of-the-art solution for person re-ID.
  s
\end{enumerate}

The rest of the paper is organized as follows. Section~\ref{sec:relatedWorks} provides an overview of the related works. In section~\ref{sec:aanet} we describe the proposed AANet framework. Experimental results are provided in sections~\ref{sec:results} and \ref{sec:results-attr}. The paper is concluded in section~\ref{sec:conclu}. 

\begin{figure}
\centering
\includegraphics[width=\linewidth]{AAM_and_Heatmap.jpg}
\caption{Comparison between the proposed AAM and class activation map generated in GFN. The AAM captures person attributes, therefore the activated areas lie mostly within the pedestrian body. The class activation map generated in GFN is influenced by the training dataset, is less dense and may include background as part of its feature map. Best viewed in color.}
\label{fig:AAM_Heatmap}
\end{figure}

\section{Related Works}
\label{sec:relatedWorks}
%\subsection{Hand-crafted methods and Deep Learning}
%Person re-ID has always been a challenging task for computer vision community. In the past, hand-crafted methods were used. For example, Ma \etal \cite{DBLP:conf/bmvc/MaSJ12} used Gabor filter and Covariance descriptors to compute the representations. The performance was way below the current methods. With the emergence of deep learning (DL), Wu \etal \cite{DBLP:conf/wacv/WuCLWYZ16} integrated hand-crafted algorithms into CNN to outperform prior works. Nowadays most researchers move away from the traditional methods totally, and fully embrace DL. 
In recent years many approaches have been explored to solve the person re-ID problem using traditional computer vision and deep learning based methods. An exhaustive overview of all person re-ID methods is out of the scope of this paper. In this section, we provide an overview of the recent deep learning based methods that achieve good performance on benchmark datasets.

Deep learning based re-ID solutions are often posed as an identity classification problem. Authors in \cite{DBLP:conf/cvpr/XiaoLOW16} used multi-domain datasets to achieve high re-ID performance in a classification based method. Wang \etal \cite{DBLP:conf/cvpr/WangZLZZ16} proposed to formulate the person re-ID problem as a joint learning framework that learns feature representations using not only the query image but also query and gallery image pairs. Many methods have used additional semantic cues such as human pose or body parts to further improve the classification performance. Su \etal \cite{DBLP:conf/iccv/SuLZX0T17} proposed a Pose-driven Deep Convolutional (PDC) model to learn improved feature extraction and matching models for end-to-end learning. Wei \etal \cite{DBLP:conf/mm/WeiZY0T17} also adopted the human pose estimation, or key point detection approach, in his Global-Local-Alignment Descriptor (GLAD) algorithm. The local body parts are detected and learned together with the global image by the four-stream CNN model, which yields a discriminatory and robust representation. Yao \etal \cite{DBLP:journals/corr/YaoZZLT17} proposed the Part Loss Networks (PL-Net) to automatically detect human parts and train them with the main identity task. Zhao \etal \cite{DBLP:conf/iccv/ZhaoLZW17} follows the concept of attention model and uses a part map detector to extract multiple body regions in order to compute their corresponding representations. The model is learnt through triplet loss function. Sun \etal \cite{Sun_2018_ECCV} proposed a strong part-based convolutional baseline method, with refined part pooling method to re-align parts for high accuracy performance. Kalayeh \etal \cite{kalayeh2018human} used multiple datasets, deep backbone architecture, large training images, and human semantic parsing to achieve good accuracy results. 

Integrating semantic information such as body parts and pose estimation have shown significant improvement in person re-ID performance. Since a person's attributes do not change significantly between the query image and the gallery images, we believe that attributes form a key information that can significantly impact person re-ID performance. This, however, has not been utilized in the current re-ID methods. In view of this, we propose to integrate attributes to the identity classification frameowrk.

%Zhou \etal \cite{zhou2016learning} proposed the Class-Activation Mapping (CAM) technique by using Global Average Pooling (GAP). CAM is not a re-ID task, but it's ability to locate objects lying within the feature map allows better representation learning in many vision tasks.
%\par Usually works adopting the human pose estimation approach require external annotations, while body part detection need no assistant from additional dataset.

%\subsection{Person attribute approach}
%Zhou \etal \cite{yin2018adversarial} used the adversarial technique to learn a semantically discriminatory joint space of a person image and generate an aligned analogous image for high level attribute image. Wang \etal \cite{wang2018transferable} proposed an unsupervised learning of transferring the the labelled information of a dataset to another unlabelled target domain for person re-id prediction. Both identity and attributes are learned and transferred. Wang \etal \cite{wang2017attribute} developed a Joint Recurrent Learning (JRL) model that is able to learn jointly attribute sequential ordering dependencies in the end-to-end encoder-decoder network.

\section{Proposed Attribute Attention Network (AANet)}
\label{sec:aanet}
%We first explained our AANet high level architecture, then we elaborate on each of the tasks. We conclude this section with loss calculation and implementation.

%\subsection{AANet Architecture Design}
The proposed AANet is a multitask network with three sub-networks, namely the GFN, PFN and AFN (Figure~\ref{fig:AANet}). The sub-network, GFN, performs global image label classification. The PFN detects and extracts localized body parts before the classification task. The AFN uses person attributes for the classification task and generates the Attribute Activation Map (AAM) that plays a crucial role in image level identity classification. All three tasks are jointly learnt resulting in a very discriminatory representation at AANet top layers. These various components of AANet are described in detail in the following sections.

\par The backbone network of AANet is based on ResNet architecture (Figure~\ref{fig:AANet}) since ResNet is known to perform well in re-ID problems. We removed the fully connected layer of the backbone network so that AANet's sub-networks can be integrated.

\subsection{Global Feature Network}
This network performs the identity classification using the global query image (Figure~\ref{fig:AANet}). The convolutional feature map $X \in R^{z\times{h}\times{w}}$ extracted by the backbone network is provided as input to a global average pooling (GAP) layer. This is followed by a 1x1 convolution layer that brings the dimensionality down to V. BatchNorm and Relu layers this convolutional layer. Finally, a fully connected layer of dimensionality C followed by softmax is appended for ID classification. 

%\begin{figure}
%\centering
%\includegraphics[width=\linewidth]{latex/images/GFN.jpg}
%\caption{GFN is the main task of AANet. It performs global ID classification. During the forward pass, the input feature map \(X\) goes through GAP, then a 1x1 convolution to reduce the channel depth from z to v, then to the fully connected layer with the dimension similar to the number of training identities. Best viewed in color}
%\label{fig:GFN}
%\end{figure}

\subsection{Part Feature Network}
This network performs identity classification on body parts using the same identity labels as used in GFN. The architecture is shown in Figure \ref{fig:PFN}. The body part detector partitions the convolutional feature map X into six horizontal regions of interest (ROIs). This is done by identifying peak activation regions in $X$. Let $(h_z, w_z)$ denote the peak activation location in each feature map $z$ of $X$ where $z\in\{1,\hdots ,Z\}$. 
\begin{equation}
(h_z,w_z) = \arg\max_{h,w}X_z(h,w)
\end{equation}
where $X_z(h,w)$ is the activation value at location $(h,w)$ on the $z$'th feature channel of $X$. These locations are then clustered into $6$ bins based on the $L_2$ distance between them. These $6$ bins constitute the $6$ ROIs/ parts. The feature map $X$ is now divided into $6$ parts using these ROIs. Figure~\ref{fig:PFN} shows this process. Once the $6$ parts are computed, the subsequent processing invovles GAP, 1x1 convolution, BatchNorm, ReLu, fully connected layer and softmax as in the GFN sub-network. 

\begin{figure}
\centering
\includegraphics[width=\linewidth]{PFN.jpg}
\caption{The PFN divides the feature map $X\in R^{Z\times{H}\times{W}}$ into six ROIs using peak activation pooling. Features from these $6$ ROIs are further used for identity classification. Best viewed in color.}
\label{fig:PFN}
\end{figure}


\begin{figure}
\centering
\includegraphics[width=\linewidth]{attr_classifiers.jpg}
\caption{The 12 attributes are generated from global, top, middle and bottom vectors on Market1501 dataset.}
\label{fig:attr_classifiers}
\end{figure}

\begin{figure*}
\centering
\includegraphics[scale=0.35]{attr_to_aam.jpg}
\caption{On Market1501 dataset, a total of 12 attention maps are used. Eight most important attributes are shown. Only six of these with strong visual cues are selected for AAM composition. Global attention map obtained from the GFN is shown here for qualitative comparison with other attributes. Backpack, handbag, bag and hat attributes, despite being important visual cues, do not appear in all images, and are therefore dropped. Note that attention map for sleeves captures too much background information and thus is unsuitable for AAM. Best viewed in color.}
\label{fig:attrs_to_aam}
\end{figure*}

\subsection{Attribute Feature Network}

The AFN is captures the key attribute information in the AANet architecture (Figure~\ref{fig:AANet}). The AFN consists of two sub-tasks (i) attribute classification and (ii) attribute attention map (AAM) composition. The first sub-task performs classification on individual person attributes. The second sub-task leverages on the output of first sub-task and generates class activation map (CAM) \cite{zhou2016learning} for each attribute. The CAMs from all attribute classes are combined to form a feature map that learns discriminatory attributes for identity classification. We describe these two sub-tasks in the following paragraphs in detail. 

\textbf{(i) Attribute classification} 
The first sub-task of AFN is to perform attribute classification. There are 10 and 12 annotated attributes on DuketMTMC-reID and Market1501 respectively. The first layer of AFN is a 1x1 convolution that downsized the channel depth of feature map X from Z to V. Next, we partition the feature maps into three different sets, namely the Top, Middle and Bottom feature maps, each responsible for extracting features form their localized regions. Part-based modeling is known to reduce background clutter and improve classification accuracy. The different parts focus on different attributes. The Top feature maps, for example, are used for capturing features such as hat, hair, sleeves and upper clothing color etc. Features from the lower half of the body are ignored in the Top feature map. As shown in Figure \ref{fig:attr_classifiers}, the outputs of these feature maps are average pooled to compute a layer of size V. The Top, Middle and Bottom feature maps are also augmented with a global feature map as shown in Figure~\ref{fig:AANet}. These four feature maps are then connected to their respective fully connected layers as shows in Figure~\ref{fig:attr_classifiers} for the respective attribute classification. 

\textbf{(ii) Attribute Attention Map} The Attribute Attenion Map (AAM) is used to perform person identity classification by combining class sensitive activation regions from individual attributes (Figure \ref{fig:AANet}). These individual class senstitive activation regions are extracted using CAM for each attribute class. Figure~\ref{fig:attrs_to_aam} shows some example of class senstive activation regions and the combined AAM. The second column in the figure shows the activation map generated by the global identification task (GFN). This activation map is shown solely for qualitative comparison. The subsequent columns show the class specific activation regions of various attributes such as gender, hair, sleeve, upper clothin color etc. The sixth column, for example, depicts the class specific activation region for upper clothing color. We can observe that the activation region corresponds to the upper clothing region in the input query image. 

\par Out of the 12 available attributes, the gender, hair, upper and lower clothing colors, lower clothing type and length are good choices for AAM composition. The AAM composition process involves averaging the individual class specific activation regions and performing an adaptive thresholding. The thresholding process removes some background regions that sometimes appear within the class specific activation region. An example of this can be observed in the second row of Figure~\ref{fig:attrs_to_aam} where the Lower clothing activation map contains some background region but on thresholding the region is removed from the composited AAM. When qualitatively comparing the class activation map generated by the global feature network on the same query image, we can see that the AAM was more specific in localizing regions with distinct attribute information.

\subsection{Loss calculation}
The proposed AANet is formulated as a multitask network. The multitask loss function of the AANet is defined as follows:
\begin{align}
%  L_{global}(y^G,d) & = %-\sum_{i=1}^{C}log(\frac{exp(y_i^G)}{\sum_{c=1}^{C}exp(y_c^G)}q(i)
    \mathcal{L}_{total}(x;\theta;\lambda) = \sum_{i=0}^{T}\lambda_i\mathcal{L}_i(x;\theta)
\end{align}
Where x is a set of training images, \(\theta\)  is the network parameters learned by minimizing \(\mathcal{L}_{total}\). \(T\) is the total number of task loss. \(\lambda_i\)'s ares the weighting factors. \(\mathcal{L}_{total}\) is thus given as
%L_total=λ_1 L_global+ λ_2 L_part+ λ_3 L_attribute		    %     (2)
\begin{align}
    \mathcal{L}_{total} = \lambda_g\mathcal{L}_{global} + \lambda_p\mathcal{L}_{part} +
    \lambda_a\mathcal{L}_{attr} + \lambda_{aam}\mathcal{L}_{aam}
\end{align}
Where \(\mathcal{L}_{global}\), \(\mathcal{L}_{part}\), \(\mathcal{L}_{attr}\) and \(\mathcal{L}_{aam}\) are the task losses of GFN, PFN and AFN (attribute classification and AAM) respectively. All task losses are computed as cross-entropy losses during training. The contribution of each loss term $(\lambda_g,\lambda_p,\lambda_{attr},\lambda_{aam})$ for optimal identity classification accuracy is automatically computed using homoscedastic uncertainty learning. 

\subsection{Implementation}

We implemented AANet with ResNet-50 and ResNet-152 as backbone networks, and pre-trained them with the ImageNet dataset. Training images are enlarged to 384 x 128, with only random ﬂip as the data augmentation method. Batch size is set to 32 for ResNet-50, and 24 for ResNet-152. Using Stochastic Gradient Descent (SGD) as the optimizer, we train the network for 40 epoch. Learning rate starts at 0.1 for the newly added layers, and 0.01 for the pretrained ResNet parameters, and follows the staircase schedule at 20 epoch with a 0.1 reduction factor for all parameters. In all the three sub-networks, the value of Z is 2048 and that of V is 256. The value of C depends on the dataset under evaluation. For DukeMTMC-reID \cite{ristani2016performance}, C is 702 and for for Market1501 \cite{DBLP:conf/iccv/ZhengSTWWT15} it is 751. 

When testing for accuracy performance, we concatenate the outputs of the V layer from all the classifiers, namely, the global identity classifier, the body part classifier, the attribute classifier and the AAM-based identity classifier (Figure~\ref{fig:AANet}) to form the representation of the query image. For ranking, we use the \(l_2\) norm between these descriptors of the query and the gallery images.

\section{Experimental Results}
\label{sec:results}
In the following experiments, we used the DukeMTMC-reID \cite{ristani2016performance} and Market1501 \cite{DBLP:conf/iccv/ZhengSTWWT15} datasets to conduct our training and testing. DukeMTMC-reID is a subset of DukeMTMC dataset. The images are cropped from videos taken from 8 cameras. The dataset consists of 16,522 training images and 17,661 gallery images, with 702 identities for both training and testing. 408 distractor IDs are also included in the dataset. There are a total of 23 attributes annotated by Lin \etal \cite{DBLP:journals/corr/LinZZWY17}. We use all attributes, but with modification to the clothing color attributes. We merged all 8 upper clothing color attributes and 7 lower clothing color attribute into a single upper clothing attribute and a single lower clothing attribute respectively. 

\par For Market1501, there are a total of 32,668 images for both training and testing. There are 751 identities allocated for training and 750 identities for testing. Lin \etal \cite{DBLP:journals/corr/LinZZWY17} also annotated this dataset, but with 27 person attributes. We use the same clothing color strategy as in DukeMTMC-reID, and use all attributes for training our model.


\subsection{Comparison with Existing Methods}

\par\textbf{DukeMTMC-reID dataset} We perform comparison with the state-of-the-art methods in Table~\ref{table:compare_duke}. The table has three parts based on the backbone network being used. First part compares models based on ResNet-50. The three comparative networks are KPM (Res-50) \cite{shen2018end}, PCB (Res-50)\cite{Sun_2018_ECCV} and the proposed AANet-50. We outperform the best state-of-the-art method \cite{Sun_2018_ECCV} in this category by 3.36\% in mAP and 3.12\% in Rank-1 accuracy.

\par The second comparison is based on networks using larger backbone models, which include both ResNet-101 and ResNet-152. The three comparitive networks are GP-reID (Res-101) \cite{almazan2018re}, SPReID (Res-152) \cite{kalayeh2018human} and the proposed AANet-101. Here, we again outperformed the state-of-the-art method \cite{kalayeh2018human} by 1.04\% in mAP and 1.79\% in Rank-1 accuracy.

\par The third comparison is based on networks from the second comparison, but this time with re-ranking \cite{DBLP:conf/cvpr/ZhongZCL17}. We outperformed the state-of-the-art method \cite{almazan2018re} by 2.05\% in mAP and 1.52\% in Rank-1 accuracy. 

\setlength{\tabcolsep}{8pt}
\begin{table}
\begin{center}
\begin{tabular}{l c c}
\hline\noalign{\smallskip}
\multicolumn{3}{c}{DukeMTMC-reID}\\
Methods & mAP & Rank-1\\
\noalign{\smallskip}
\hline
\noalign{\smallskip}
%LOMO+XQDA \cite{DBLP:conf/cvpr/LiaoHZL15} & 17.0 & 30.8\\
%GAN	\cite{DBLP:conf/iccv/ZhengZY17} & 47.1 & 67.7\\
%APR \cite{DBLP:journals/corr/LinZZWY17} & 51.9 & 70.7\\
%PAN	\cite{DBLP:journals/corr/ZhengZY17aa} & 51.5 & 71.6\\
FMN \cite{DBLP:journals/corr/abs-1711-07155} & 56.9 & 74.5\\
SVDNet \cite{DBLP:conf/iccv/SunZDW17} & 56.8 & 76.7\\
DPFL \cite{DBLP:conf/iccvw/ChenZG17} & 60.6 & 79.2\\
\hline
KPM (Res-50) \cite{shen2018end} & 63.2 & 80.3\\
PCB (Res-50)\cite{Sun_2018_ECCV} & 69.2 & 83.3\\
{\bf Proposed AANet-50}	& {\bf72.56} & {\bf86.42}\\
\hline
GP-reID (Res-101) \cite{almazan2018re} * & 72.80 & 85.20 \\
SPReID (Res-152) \cite{kalayeh2018human} & 73.34 & 85.95 \\ 
{\bf Proposed AANet-152}	& {\bf74.38} & {\bf87.74}\\
\hline
GP-reID (Res-101)\cite{almazan2018re} + RR * & 85.60 & 89.40 \\
SPReID (Res-152)\cite{kalayeh2018human} + RR & 84.99 & 88.96 \\ 
{\bf Proposed AANet-152 + RR} & {\bf87.04} & {\bf90.48}\\
\hline
\end{tabular}
\end{center}
\caption{Performance comparison with other state-of-the-art methods using DukeMTMC-reID dataset. AANet-50 denotes AANet trained using ResNet-50. AANet-101 denotes AANet trained using ResNet-101. RR deonotes Re-Ranking\cite{DBLP:conf/cvpr/ZhongZCL17}
\label{table:compare_duke}. * indicates methods published only in arXiv.}
\end{table}
\setlength{\tabcolsep}{1.4pt}

\par \textbf{Market1501 dataset} We perform similar comparisons as in previous section in Table~\ref{table:compare_market1501} using the Market1501 dataset. In the first comparison, which uses ResNet-50, the networks selected are KPM (Res-50) \cite{shen2018end}, PCB (Res-50)\cite{Sun_2018_ECCV} and the proposed AANet-50. We outperformed the best state-of-the-art method \cite{Sun_2018_ECCV} in this category by 0.8\% in mAP and 0.07\% in Rank-1 accuracy.

\par The second comparison is made using GP-reID (Res-101) \cite{almazan2018re}, SPReID (Res-152) \cite{kalayeh2018human} and the proposed AANet, with either ResNet-101 or ResNet152. Here, we again outperformed the state-of-the-art method \cite{kalayeh2018human} by 0.05\% in mAP and 0.25\% in Rank-1 accuracy.

\par The third comparison is made on networks from the previous section but with re-ranking~\cite{DBLP:conf/cvpr/ZhongZCL17}. We outperform the state-of-the-art method \cite{kalayeh2018human} by 1.42\% in mAP and 0.47\% in Rank-1 accuracy. We believe that the attribute information is a key contributor in AANet's person re-ID performance.

\setlength{\tabcolsep}{1pt}
\begin{table}
\begin{center}
\begin{tabular}{l c c c c}
\hline\noalign{\smallskip}
\multicolumn{5}{c}{Market1501}\\
Methods & mAP & Rank1 & Rank5 & Rank10\\
\noalign{\smallskip}
\hline
\noalign{\smallskip}
%PAR \cite{DBLP:conf/iccv/ZhaoLZW17} & 63.4 & 81.0 & 92.0 & 94.7\\
%MultiLoss \cite{DBLP:conf/ijcai/LiZG17} & 64.4 & 83.9 & - & -\\
%PDC \cite{DBLP:conf/iccv/SuLZX0T17} & 63.4 & 84.4 & 92.7 & 94.9\\
PL-Net \cite{DBLP:journals/corr/YaoZZLT17} & 69.3 & 88.2 & - &	-\\
DPFL \cite{DBLP:conf/iccvw/ChenZG17} & 73.1 & 88.9	& -	& -\\
GLAD \cite{DBLP:conf/mm/WeiZY0T17} & 73.9 & 89.9 & - & -\\
\hline
KPM (Res-50)\cite{shen2018end} & 75.3 & 90.1 & 96.7 & 97.9\\
PCB (Res-50)\cite{Sun_2018_ECCV} & 81.6 & 93.8 & 97.5 & 98.5\\
{\bf Proposed AANet-50} & {\bf82.40} & {\bf93.87} & {\bf97.61} & {\bf98.56}\\
\hline
GP-reID (Res-101) \cite{almazan2018re}* & 81.20 & 92.20 & \bf97.90 & - \\
SPReID (Res-152) \cite{kalayeh2018human} & 83.36 & 93.68 & 97.57 & 98.40 \\ 
{\bf Proposed AANet-152} & {\bf83.41} & {\bf93.93} & {97.64} & {\bf98.53}\\
\hline
GP-reID (Res-101)\cite{almazan2018re}+RR* & 90.00 & 93.00 & 95.90 & - \\
SPReID (Res-152)\cite{kalayeh2018human}+RR & 90.96 & 94.63 & 96.82 & 97.65 \\ 
{\bf Proposed AANet-152+RR} & {\bf92.38} & {\bf95.10} & {\bf97.32} & {\bf97.94}\\
\hline
\end{tabular}
\end{center}
\caption{Performance comparison with other state-of-the-art methods using Market1501 dataset. AANet-50 denotes AANet trained using ResNet-50. AANet-152 denotes AANet trained using ResNet-152. RR denotes  Re-Ranking\cite{DBLP:conf/cvpr/ZhongZCL17}. * indicates methods published only in arXiv.
 }
\label{table:compare_market1501}
\end{table}
\setlength{\tabcolsep}{1.4pt}

\subsection{Network Design and Analysis}
In this section, we study the effect of input image size and the size of the backbone network on the re-ID performance. We will also review the design strategies that effects the attribute attention map.

\par \textbf{Ablation Study} In Table \ref{table:duke_ablation_study}, we show the impact of the task loss weights on AANet accuracy performance using DukeMTMC-reID dataset. The glocal ID task, the part task, the attribute classification task and the attribute attention map task are denoted as \(\mathcal{L}_g\), \(\mathcal{L}_p\), \(\mathcal{L}_a\) and \(\mathcal{L}_{aa}\) respectively. 
As we add each of these relevant tasks to the network, the accuracy improves, which justifies the contribution of each task on the overall performance. When we use homoscedastic uncertainty learning to obtain the task loss weights \(\mathcal{L}_g\), \(\mathcal{L}_p\) and \(\mathcal{L}_a\), the performance improves to 70.47\% mAP and 85.44\% Rank-1 accuracy. This result alone is enough to outperform the best state-of-the-art method using ResNet-50. With the integration of AAM, we improve the accuracy result to 72.56\% mAP and 86.42\%. 

\par \textbf{Effect of Backbone Network} As shown by Kalayeh \etal \cite{kalayeh2018human} and Almazan \etal \cite{almazan2018re}, the depth of the backbone network affects the accuracy performance of person re-ID. Deeper networks yield better result, and this is clearly shown in both Tables \ref{table:compare_duke} and \ref{table:compare_market1501}. Table \ref{table:compare_duke} shows that the proposed AANet-50 outperformed SPReID (Res-152) \cite{kalayeh2018human} in Rank-1 accuracy by 0.47\%, and GP-reID (Res-101) \cite{almazan2018re} by 1.22\%. We achieved similar Rank-1 results on Market1501 dataset also, with our AANet-50 outperforming those using deeper backbone networks. 

\par \textbf{Effect of Training Parameters} Many tricks have been used in the literature to enhance accuracy \cite{kalayeh2018human} and \cite{almazan2018re}. In \cite{kalayeh2018human}, the authors aggregate a total of 10 different datasets to generate $\sim$ 111k images and $\sim$ 17k identities for training and testing. In addition, multiple image sizes are used to train the network in different phases. In \cite{almazan2018re}, authors use techniques such as pre-training before regression learning, large image size, hard triplet mining and deeper backbone network for good person re-ID. The proposed AANet uses smaller image size, simpler training process, and a shallower ResNet-50 arechitecture to outperform existing state-of-the-art.
%mention about X dimension, number of parts
%Thresholding for both part and attribute

\setlength{\tabcolsep}{4pt}
\begin{table}
\begin{center}
\begin{tabular}{ | l | C{0.3cm} | C{0.3cm} | C{0.3cm} | C{0.3cm} | C{0.85cm} | C{0.85cm} |}
\hline%\noalign{\smallskip}
%\multicolumn{1}{l|}{} & \multicolumn{3}{c|}{} & %\multicolumn{2}{c|}{Classification} & \multicolumn{1}{c}{}\\
%\multicolumn{1}{|l|}{} & \multicolumn{3}{c|}{} & \multicolumn{2}{c|}{Accuracy}\\
%\cline{5-6}
\multicolumn{1}{|l|}{AANet-50} & \multicolumn{4}{c|}{Task} & \multicolumn{1}{c|}{mAP} & \multicolumn{1}{c|}{Rank 1}\\
\multicolumn{1}{|l|}{Task Loss} & \multicolumn{4}{c|}{Weights} & \multicolumn{1}{c|}{\%} & \multicolumn{1}{c|}{\%}\\
\hline
\(\mathcal{L}_g\) & 1 & 0 & 0 & 0 & 62.92 & 80.18\\
%\(\mathcal{L}_p\) & 0 & 1 & 0 & 74.3 & 91.0\\
%\(\mathcal{L}_a\) & 0 & 0 & 1 & - & -\\
%\(\mathcal{L}_g + \mathcal{L}_a\) & 1 & 0 & 1 & 75.5 & 90.3\\
\(\mathcal{L}_g + \mathcal{L}_p\) & 1 & 1 & 0 & 0 & 66.35 & 82.93\\
\(\mathcal{L}_g + \mathcal{L}_p + \mathcal{L}_a\) & 1 & 1 & 1 & 0 & 67.28 & 83.29\\
\hline
\multicolumn{1}{|l|}{\(\mathcal{L}_g + \mathcal{L}_p\ + \mathcal{L}_a\)} & \multicolumn{4}{c|}{Uncertainty} & \multicolumn{1}{c|}{70.47} & \multicolumn{1}{c|}{85.44}\\
\multicolumn{1}{|l|}{\(\mathcal{L}_g + \mathcal{L}_p + \mathcal{L}_a + \mathcal{L}_{aa}\)} & \multicolumn{4}{c|}{Learning} & \multicolumn{1}{c|}{\textbf{72.56}} & \multicolumn{1}{c|}{\textbf{86.42}}\\
\hline
\end{tabular}
\end{center}
\caption{Performance comparisons of different combination of task losses using DukeMTMC-reID dataset, with and without uncertainty learning. The top three rows are AANet accuracy with equal weights to the tasks. Bottom two rows show the results with loss weights obtained from uncertainty learning.
}
\label{table:duke_ablation_study}
\end{table}
\setlength{\tabcolsep}{1.4pt}

\begin{figure}
\centering
\includegraphics[width=\linewidth]{Image_retrieval_good.jpg}
\caption{Three queries from the DukeMTMC-reID with eight retrieved images for each query.}
\label{fig:good_retrieval}
\end{figure}


\begin{figure*}
\centering
\includegraphics[width=\linewidth]{attr_query.jpg}
\caption{Three examples of how person attributes help in improving the image retrieval accuracy. First row used gender and color attributes to filter the retrieved images to get correct images within the top 5 ranks. Second row used hat, color and gender attributes to achieve same result as first row. Last row used color and backpack attributes to filter away falsely accepted images. Green box denotes same ID as query image. Red box denotes different ID from query image. Best viewed in color}
\label{fig:attr_query}
\end{figure*}

\setlength{\tabcolsep}{4pt}
\begin{table*}
\begin{center}
\begin{tabular}{ l | c c c c c c c c c c c c | c }
\hline
Methods & gender & age & hair & L.slv & L.low & S.clth & B.pack & H.bag & bag & hat & C.up & C.low & mean\\
\hline
APR \cite{DBLP:journals/corr/LinZZWY17} & 86.45 & 87.08 & 83.65 & 93.66 & 93.32 & 91.46 & 82.79 & 88.98 & 75.07 & 97.13 & 73.40 & 69.91 & 85.33\\
AANet-152 & {\bf92.31} & {\bf88.21} & {\bf86.58} & {\bf94.45} & {\bf94.24} & {\bf94.83} & {\bf87.77} & {\bf89.61} & {\bf79.72} & {\bf98.01} & {\bf77.08} & {\bf70.81} & {\bf87.80}\\
\hline
\end{tabular}
\end{center}
\caption{Performance comparisons of attribute accuracy on Market1501 dataset.
}
\label{table:attr_accuracy}
\end{table*}
\setlength{\tabcolsep}{1.4pt}

\section{Experimental Results using Attributes}
\label{sec:results-attr}
In this section, we illustrate how person attributes help in refining the retrieved images for image-based person re-ID. 

\subsection{Retrieval results}
We show three retrieval examples using AANet in Figure \ref{fig:good_retrieval}. Though there are some occlusions on the query subjects, for examples, tree, cars and unwanted pedestrian, AANet successfully retrieves correct images from the gallery set.
\par In Figure~\ref{fig:attr_query}, we show some examples of challenging queries where the subjects are heavily occluded. This resulted in poor retrieval accuracy. The figure demonstrates that person attributes helps to filter out the incorrect retrievals. Three examples are given, each with their own retrieval difficulties. First example is given in row one. More than half of the query subject is occluded, and the upper clothing color was similar to the other pedestrian clothing. Out of the top 10 images retrieved, only one correct image was retrieved. To filter away the wrong identities, we use person attribute query, by specifying male and white lower clothing color attributes as search criteria, and compare them with the predicted attributes of the retrieved images. AANet successfully returns correct identity images within the top 5 ranks. In the second row, the query subject is the lady in green and red clothing, but the retrieved images point to identities wearing white clothing only. The correct images are actually ranked from 14 to 21. To get the right images, we specified green and red clothing color attributes, gender attribute and hat attribute to effectively remove all those false retrievals, leaving us the images from correct identity. In last row, the subject is severely occluded, and has very similar attributes as found in those incorrect retrievals. We relied on black and gray clothing colors, and backpack attributes to retrieve all correct images within the top 5 rank.

\subsection{Attribute Classification Performance}
The accuracy of attribute classification of the proposed AANet is compared with APR \cite{DBLP:journals/corr/LinZZWY17} in Table \ref{table:attr_accuracy}. APR \cite{DBLP:journals/corr/LinZZWY17} is provided by Lin \etal, the author who annotated the DukeMTMC-reID and Market1501 datasets with person attributes. As shown in the table, AANet outperforms APR in classifying all the attributes. %It is worth noting that color related attributes, like the upper and lower clothing colors, do not perform well for both networks when compared to the rest of the attributes. The reason being cameras used to take videos or images are not color calibrated after installation. 
%Nonetheless, it is still very handy when performing image retrieval. 

%\setlength{\tabcolsep}{8pt}
%\begin{table}
%\begin{center}
%\begin{tabular}{l c c}
%\hline\noalign{\smallskip}
%\multicolumn{3}{c}{ResNet-50 AAM Design Parameters}\\
%Methods & mAP & Rank-1\\
%\noalign{\smallskip}
%\hline
%\noalign{\smallskip}
%\hline
%1 vector + no threshold  & 81.99 & 93.50 \\
%1 vector + threshold & 82.04 & 93.48 \\ 
%\hline
%4 vectors + no threshold  & 81.89 & 93.42 \\
%4 vectors + threshold & {\bf82.40} & {\bf93.87} \\
%\hline
%\end{tabular}
%\end{center}
%\caption{Performance comparison on AAM design parameters.}
%\label{table:aam_design_para}
%\end{table}
%\setlength{\tabcolsep}{1.4pt}

%\subsection{ResNet-50 AAM design parameters}
%We tested two crucial AAM parameters to validate our design assumptions. The first is the number of vectors used to generate the attributes. We tested single global vector vs the 4 global, top, middle and bottom vectors. We also tested the effectiveness of thresholding the AAM. The results are shown in Table \ref{table:aam_design_para}, which confirms that global and localized region vectors, and thresholding AAM give the best result. These parameters, in reality, reduce unwanted noise from our intended features, thus allowing our AANet to learn better.



\section{Conclusions}
\label{sec:conclu}
%We showed that our AANet, with the attribute attention map capturing the class sensitive regions, and attenuating the backgrounds, is able to share its unique learning experience with the global identity task, and compliment each others to bring out the very discriminatory features useful for person re-ID task. As a result, we outperformed the best state-of-of-art methods, regardless of the backbone architecture employed. On top of that, our AANet achieves good accuracy on person attribute prediction. This provides our user a very efficient and flexible image retrieval system.
%\par One area which we think we can pursue in the future is to leverage on those under utilized attributes to create a more complete person attention map.
In this paper we propose a novel architecture to incorporate attributes based on physical appearance such as clothing color, hair, presence/absence of backpack etc. into a classification based person re-id framework. The propsosed Attribute Attenion Network (AANet) employs joint end-to-end learning and homoscedastic uncertainty learning for multitask loss fusion. The resulting network outperforms existing state-of-the-art re-id methods on multiple benchmark datasets. 
{\small
\bibliographystyle{ieee}
\bibliography{egbib}
}
%\end{multicols}
\end{document}


==> AANet_cvpr2019_v7.tex <==
%\documentclass[10pt,twocolumn,letterpaper]{article}

%\documentclass[10pt,letterpaper]{article}
%\usepackage{multicol}

\usepackage{cvpr}
\usepackage{times}
\usepackage{epsfig}
\usepackage{graphicx}
\usepackage{amsmath}
\usepackage{amssymb}

\usepackage{array}
\newcolumntype{L}[1]{>{\raggedright\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\newcolumntype{C}[1]{>{\centering\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\newcolumntype{R}[1]{>{\raggedleft\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}

% Include other packages here, before hyperref.

% If you comment hyperref and then uncomment it, you should delete
% egpaper.aux before re-running latex.  (Or just hit 'q' on the first latex
% run, let it finish, and you should be clear).
\usepackage[pagebackref=true,breaklinks=true,letterpaper=true,colorlinks,bookmarks=false]{hyperref}

% \cvprfinalcopy % *** Uncomment this line for the final submission

\def\cvprPaperID{4013} % *** Enter the CVPR Paper ID here
\def\httilde{\mbox{\tt\raisebox{-.5ex}{\symbol{126}}}}

% Pages are numbered in submission mode, and unnumbered in camera-ready
\ifcvprfinal\pagestyle{empty}\fi
\begin{document}

%%%%%%%%% TITLE
\title{AANet: Attribute Attention Network for Person Re-Identifications}

\author{First Author\\
Institution1\\
Institution1 address\\
{\tt\small firstauthor@i1.org}
% For a paper whose authors are all at the same institution,
% omit the following lines up until the closing ``}''.
% Additional authors and addresses can be added with ``\and'',
% just like the second author.
% To save space, use either the email address or home page, not both
\and
Second Author\\
Institution2\\
First line of institution2 address\\
{\tt\small secondauthor@i2.org}
}

\maketitle
%\thispagestyle{empty}

%\begin{multicols}{2}

%%%%%%%%% ABSTRACT
\begin{abstract}
   %The ABSTRACT is to be in fully-justified italicized text, at the top
   %of the left-hand column, below the author and affiliation
   %information. Use the word ``Abstract'' as the title, in 12-point
   %Times, boldface type, centered relative to the column, initially
   %capitalized. The abstract is to be in 10-point, single-spaced type.
   %Leave two blank lines after the Abstract, then begin the main text.
   %Look at previous CVPR abstracts to get a feel for style and length.
   
   %In this paper, we propose a new person re-identification (re-ID) method by using person attributes, and by learning the merged regions indicated by class sensitive localized neuron responses from individual attributes, to assist the main identity classification task. We call this the  Attribute Attention Network (AANet). A person re-ID model usually requires additional cues, such as body parts or human pose estimation to enhance the prediction job. We built our baseline network using the same concept. Our AANet consists of the main identification task with a sub task to detect body parts. We then integrate a crucial attribute detection task, which extracts class sensitive regions for learning. We believe that there are many useful features hidden within the Convolutional Neural Network (CNN). By searching for class aware responses of the individual attributes and combining them to form the attribute attention map (AAM), we arrived at a person re-ID network that has very strong discriminatory representations. When benchmark against the work done by Sun \etal \cite{Sun_2018_ECCV}, which is the best state-of-the-art method with ResNet-50, we outperform it by 3.36\% mAP and 3.12\% Rank-1 accuracy on DukeMTMC-reID dataset. On the Market1501 dataset, we outperform the same work by 0.8\% mAP and 0.08\% Rank-1 accuracy. We also outperform other state-of-the-art methods utilizing deeper backbone architectures. Our AANet, trained with ResNet-152, achieves 92.38\% mAP and 95.10\% Rank-1 in re-rank accuracy. Furthermore, we have the ability to predict person attribute, giving our user a flexible and powerful text-based query system for person image retrieval.
   
   This paper proposes Attribute Attention Network (AANet), a new architecture that integrates person attributes and attribute attention maps into a classification framework to solve the person re-identification (re-ID) problem. Many person re-ID models typically employ semantic cues such as body parts or human pose to improve the re-ID performance. Attribute information, however, is often not utilized. The proposed AANet leverages on a baseline model that uses body parts and integrates the key attribute information in an unified learning framework. The AANet consists of a global person ID task, a part detection task and a crucial attribute detection task. By estimating the class responses of individual attributes and combining them to form the attribute attention map (AAM), a very strong discriminatory representation is constructed. The proposed AANet outperforms the best state-of-the-art method \cite{Sun_2018_ECCV} by 3.36\% in mAP and 3.12\% in Rank-1 accuracy on DukeMTMC-reID dataset. On Market1501 dataset, AANet achieves 92.38\% mAP and 95.10\% Rank-1 with re-ranking thus outperforming~\cite{Sun_2018_ECCV} by 0.8\% in mAP and 0.08\% in Rank-1 accuracy. We also outperform other state-of-the-art methods utilizing deeper backbone architectures. In addition, AANet can perform person attribute prediction (e.g., gender, hair length, clothing length etc.), and generate text-based descriptions of the attributes together with their heat maps. This enables text-based query for person image retrieval further complementing the existing image-based person re-ID approaches.
   
\end{abstract}

%%%%%%%%% BODY TEXT
\section{Introduction}

%Conventionally, person re-ID aims to retrieve images of a person taken from an array of cameras, or from same camera but from different occasions, by using a query image. Usually this prediction task is limited to a short time frame and within a small geographical area. This seemingly simple recognition task to human is a challenge to the machine, as factors like person occlusions, pose variation, ambient light changes, low image resolution, etc. degrade image quality and reduce effective number of usable pixels for image processing. In recent years, deep learning has overcome many limitations, and improves the retrieval performance significantly. Still, there are many rooms for improvement.

Given a query image, person re-ID aims to retrieve images of a queried person from a collection of images. The retrieval is typically attempted from a collection of images taken within a short time interval with respect to the queried image. This supports the underlying assumption that the query peron's appearance and clothing attributes remain unchanged across the query and the collection images. Person re-ID is a challenging problem due to many factors such as partial/total occlusion of the subject, pose variation, ambient light changes, low image resolution, etc. Recent deep learning based re-ID solutions have demonstrated encouraging retrieval performance. 

%\par One important person re-ID application is in the camera surveillance domain. Tens of thousands of cameras are being installed in cities all over the world, and these cameras are expected to not just record videos, but also perform identification of person attribute. Some examples of useful person attribute information are gender, hair, hat, clothing colors and types and carried bags. This prediction ability, however, is lacking in most person re-ID network.

\begin{figure}
\centering
\includegraphics[width=\linewidth]{latex/images/merged_attributes_id33.jpg}
\caption{Class-aware attribute attention maps are extracted and combined together to form a discriminatory feature map at the image level. The six attention maps shown in the figure correspond to the six attributes such as hair, upper clothing color, lower clothing color etc. Best viewed in color.}
\label{fig:MergedAttribute}
\end{figure}

\begin{figure*}
\centering
\includegraphics[width=\linewidth]{latex/images/AANet_v3.jpg}
\caption{Overview of AANet. The backbone network is based on the ResNet50 architecture. The backbone network outputs the feature map \(X\). The feature map \(X\) is forwarded to three tasks, namely the Global Feature Network(GFN), Part Feature Network (PFN) and Attribute Feature Network (AFN). The output of these three tasks are combined using uncertainty learning to predict the person identification. Best viewed in color.}
\label{fig:AANet}
\end{figure*}


%\par In this work, we aim for good person re-ID performance with person attribute prediction capability. To achieve our goals, we look to multitask network, with a person identification (ID) main task, and two relevant  attribute and body part detection sub tasks. The main task performs global feature learning. The two sub tasks, however, perform localized and different feature learning. By sharing their learning experience with the main task, we have a very discriminatory representations at the output of the network. This is shown in Figure \ref{fig:AANet}. AANet consists of two main networks. The first main network performs global identity classification, and body part detection and classification. This two tasks are managed by the Global Feature Network (GFN) and the Part Feature Network (PFN). The second main network is the Attribute Feature Network (AFN), which also consists of two tasks, namely the person attribute classification and AAM classification. All four tasks utilizes Softmax classification outputs, using image labels and person attribute labels as ground truth for learning. To ensure optimal performance, we use uncertainty learning to obtain the weighting for each task. The final task loss is then the summation of the scaled task losses.

\par The approaches used to solve the person re-ID problem can be broadly divided into two categories. The first category comprises of methods that attempt to learn an embedding space which brings images belonging to a unique person close together and those belonging to different persons far away. Various distance metrics such as triplet and quadruplet losses have been employed to learn such embedding spaces \cite{DBLP:journals/corr/HermansBL17, chen2017beyond}.

\par The second category of solutions poses the re-ID problem in a classiﬁcation set-up. Such approaches attempt to recognize the identiﬁcation of the person based on the query image using classical classiﬁcation loss functions such as cross-entropy. Research has shown that by integrating semantic information such as body parts, human pose etc, the classiﬁcation and recognition accuracy can be signiﬁcantly improved \cite{DBLP:conf/iccv/SuLZX0T17, DBLP:conf/mm/WeiZY0T17, DBLP:journals/corr/YaoZZLT17}. Person attributes, such as clothing color, hair, presence/absence of backpack, etc. are, however, not used by the current state-of-the-art re-ID solutions. Since, a typical re-ID set-up assumes that the physical appearance of the person under investigation would not significantly change between query image and the search images, physical appearance becomes a key information that can be mined to achieve higher re-ID performances. Such information is not utilized by current research and the state of the art re-ID solutions. 
\par In this work, we propose to utilize the person attribute information and integrate attribute analytics into a classiﬁcation framework to solve the re-ID problem. The resulting framework, called the Attribute Attention Network (AANet), brings together identity classiﬁcation, body part detection and person attribute analytics into an uniﬁed framework that jointly learns a highly discriminatory feature space. The resulting re-ID accuracy outperforms existing state of the art solutions in multiple benchmark datasets.  
%\par We believe that there are many discriminatory features hidden within our AANet. Object discovery with deep neural networks has been shown by Le \etal \cite{le2013building} in an unsupervised way in 2013. Zhou \etal \cite{zhou2014object} showed that for a CNN trained for scene recognition, the object detection with no supervision emerges even more than that trained with ImageNet. When the CNN is setup for scene classification with supervision, many more object can be discovered than in object classification. Inspired by this, we set out to treat our person attributes as objects and the global image as scene. We use Class-Activation Mapping (CAM) \cite{zhou2016learning} as object detector to localize the regions belonging to the person attributes. Only those attributes which exhibit strong visual cue of the human subject are combined to form a map with strong discriminatory features. This idea is shown in Figure \ref{fig:MergedAttribute}. We are not performing semantic segmentation, and thus not expecting the map to resemble fully that of the input person image. However, we can see from Figure \ref{fig:MergedAttribute} that the produced combined map gives us strong discriminatory features very useful for learning. The spatial information of the attribute objects, and their spatial relationships to each others are well captured. In addition, the background clutters are removed in most cases. This renders a more generalized network. A comparison between the AAM and global ID heat map are shown in Figure \ref{fig:AAM_Heatmap}. The AAM map follows more closely to the pedestrian shape, whereas the global ID heat map reveals whatever regions that the trained network thinks are discriminatory for ID classification, which explains why ID classification alone tends to over-fit. Thus, AAM as a relevant task in a multitask network, shares its learning experience and helps to regularize the main task.

\par Figure \ref{fig:AANet} gives an overview of the proposed architecture. The proposed framework consists of three sub-networks. The first network, called the Global Feature Network (GFN), performs global identity classiﬁcation. The second network, called the Part Feature Network (PFN), focuses on body part detection and classiﬁcation based on body parts. The third network is the Attribute Feature Network (AFN), which extracts information from the person’s physical attributes. The three networks perform Softmax classiﬁcation using image based labels and person attribute labels. We use uncertainty learning to optimize the weights of the three sub-tasks for ﬁnal loss calculations.

\par Since AANet performs person attribute classification as part of solving the re-id problem, AANet also produces text-based attribute descriptions for each query image. This enables text-based query processing in addition to the traditional image-based query processing in the re-id set-up. To the best of our knowledge, AANet is the first framework that integrates image-based and text-based query processing for person re-ID.

\par Our key contributions can be summarized as follows:
\begin{enumerate}
    \item We provide a new network architecture that integrates attribute analytics with identity and body part classification in a uniﬁed learning framework.

    \item We outperform the existing best state-of-the-art re-ID method on multiple benchmark datasets and propose the new state of the art solution for person re-ID.
    
    \item We propose the first integrated re-ID framework that supports both image and text-based query processing for re-ID.
\end{enumerate}

The rest of the paper is organized as follows. Section~\ref{sec:relatedWorks} provides an overview of the related works. In section~\ref{sec:aanet} we describe the proposed AANet framework. Experimental results are provided in section~\ref{sec:results} and the paper is concluded in section~\ref{sec:conclu}. 

\begin{figure}
\centering
\includegraphics[width=\linewidth]{latex/images/AAM_and_Heatmap.jpg}
\caption{Comparison between AAM and class activation map generated in GFN. The AAM captures person attributes, therefore the activated areas lie mostly within the pedestrian body. The class activation map generated in GFN is influenced by the training dataset, is less dense and may include background as part of its feature map. Best viewed in color.}
\label{fig:AAM_Heatmap}
\end{figure}

\section{Related works}
\label{sec:relatedWorks}
%\subsection{Hand-crafted methods and Deep Learning}
%Person re-ID has always been a challenging task for computer vision community. In the past, hand-crafted methods were used. For example, Ma \etal \cite{DBLP:conf/bmvc/MaSJ12} used Gabor filter and Covariance descriptors to compute the representations. The performance was way below the current methods. With the emergence of deep learning (DL), Wu \etal \cite{DBLP:conf/wacv/WuCLWYZ16} integrated hand-crafted algorithms into CNN to outperform prior works. Nowadays most researchers move away from the traditional methods totally, and fully embrace DL. 
In recent years many approaches have been explored to solve the re-ID problem using traditional computer vision and deep learning based methods. In this section, we provide an overview of the recent deep learning based methods that achieve close to state-of-the-art performance.

Deep learning based re-ID solutions are often posed as an identity classification problem. Authors in \cite{DBLP:conf/cvpr/XiaoLOW16} used multi-domain datasets to achieve high re-ID performance in a classification set-up. Wang \etal \cite{DBLP:conf/cvpr/WangZLZZ16} proposed to formulate the re-ID problem as a joint learning framework that learns feature representations using not only the query image but also query and gallery image pairs. Many solutions have used additional semantic cues such as human pose or body parts to further improve the classification performance. Su \etal \cite{DBLP:conf/iccv/SuLZX0T17} proposed a Pose-driven Deep Convolutional (PDC) model to learn improved feature extraction and matching models from end-to-end. Wei \etal \cite{DBLP:conf/mm/WeiZY0T17} also adopted the human pose estimation, or key point detection approach, in his Global-Local-Alignment Descriptor (GLAD) algorithm. The local body parts are detected and learned together with the global image by the four-stream CNN model, which yields a discriminatory and robust representation. Yao \etal \cite{DBLP:journals/corr/YaoZZLT17} proposed the Part Loss Networks (PL-Net) to automatically detect human parts and cross train them with the main identity task. Zhao \etal \cite{DBLP:conf/iccv/ZhaoLZW17} follows the concept of attention model and uses a part map detector to extract multiple body regions in order to compute their corresponding representations. The model is learnt through triplet loss function. Sun \etal \cite{Sun_2018_ECCV} proposed a strong Part-based Convolutional Baseline method, with Refined Part Pooling method to re-align parts for high accuracy performance. Kalayeh \etal \cite{kalayeh2018human} used multiple datasets, deep backbone architecture, large training images, and human semantic parsing to achieve good accuracy results. 

Semantic information such as body parts and pose estimation have shown significant improvement in re-ID performance. Since the physical appearance of the queried subject does not change significantly between the query image and the gallery images, we believe that physical appearance is also a key information that can significantly impact person re-ID. This, however, has not been utilized in the current re-ID solutions. In view of this, we propose to integrate physical attributes to the identity classification frameowrk.

%Zhou \etal \cite{zhou2016learning} proposed the Class-Activation Mapping (CAM) technique by using Global Average Pooling (GAP). CAM is not a re-ID task, but it's ability to locate objects lying within the feature map allows better representation learning in many vision tasks.
%\par Usually works adopting the human pose estimation approach require external annotations, while body part detection need no assistant from additional dataset.

%\subsection{Person attribute approach}
%Zhou \etal \cite{yin2018adversarial} used the adversarial technique to learn a semantically discriminatory joint space of a person image and generate an aligned analogous image for high level attribute image. Wang \etal \cite{wang2018transferable} proposed an unsupervised learning of transferring the the labelled information of a dataset to another unlabelled target domain for person re-id prediction. Both identity and attributes are learned and transferred. Wang \etal \cite{wang2017attribute} developed a Joint Recurrent Learning (JRL) model that is able to learn jointly attribute sequential ordering dependencies in the end-to-end encoder-decoder network.

\section{Proposed Attribute Attention Network (AANet)}
\label{sec:aanet}
%We first explained our AANet high level architecture, then we elaborate on each of the tasks. We conclude this section with loss calculation and implementation.

%\subsection{AANet Architecture Design}
The proposed AANet is a multitask network with three sub-networks, namely the GFN, PFN and AFN (Figure~\ref{fig:AANet}). The sub-network, GFN, performs global image label classification. The PFN detects and extracts localized body parts before the classification task. The AFN uses person attributes for the classification task and employs class activation map (CAM)~\cite{zhou2016learning} to generate the crucial Attribute Activation Map (AAM). The AAM is then used for image label classification. All three tasks are jointly learnt resulting in a very discriminatory representation at AANet top layers. These various components of AANet are described in detail in the following sections.

\par The backbone network of AANet is based on ResNet-50 architecture since ResNet is known to perform well for re-ID problems. We removed the fully connected layer of ResNet-50 so that we can integrate AANet's sub-networks. We also reduce the stride from 2 to 1 in Conv5 so that we have higher resolution for feature map X. Some works have increased the input image size to compute fine feature map X~\cite{Sun_2018_ECCV, kalayeh2018human}. Large input image sizes slow down the training. 

We have also evaluated AANet using ResNet-101 and ResNet-152 to benchmark against the state-of-the-art methods \cite{kalayeh2018human, almazan2018re} utilizing deeper backbone architectures. The results are shown in section~ref{sec:results}.

\subsection{Global Feature Network}
This network performs the identity classification using the global person image (Figure~\ref{fig:AANet}). The feature map X extracted by the backbone network is provided as input to a global average pooling (GAP) layer. This is followed by two layers called Z and V that perform 1x1 convolution to reduce the channel depth from 2048 to 256. BatchNorm and Relu layers follow the V layer. Finally, a fully connected layer C is appended for ID classification. The dimension of the layer C depends on the dataset under evaluation, for DukeMTMC-reID \cite{ristani2016performance} the size of C is 702 and for for Market1501 \cite{DBLP:conf/iccv/ZhengSTWWT15} it is 751. The GFN is optimized using a cross-entropy loss function. 

%\begin{figure}
%\centering
%\includegraphics[width=\linewidth]{latex/images/GFN.jpg}
%\caption{GFN is the main task of AANet. It performs global ID classification. During the forward pass, the input feature map \(X\) goes through GAP, then a 1x1 convolution to reduce the channel depth from z to v, then to the fully connected layer with the dimension similar to the number of training identities. Best viewed in color}
%\label{fig:GFN}
%\end{figure}

\subsection{Part Feature Network}
This network performs ID classification on body parts using the same identity labels as used in GFN. The architecture is shown in Figure \ref{fig:PFN}. The body part detector works by partitioning the feature map X into six horizontal strips. It searches for the peak neuron responses in all the z maps belonging to X. These peak responses are noted for their position within X, sorted based on their vertical position, and grouped into six bins. Each of these bins are averaged and threshold. The boundary of the threshold features, or ROIs are then calculated. With the helps of these ROIs, the feature map X can now be partitioned into 6 parts for further learning. This is shown as the rightmost image of Figure \ref{fig:PFN}, which is the extrapolation of partitioned feature map back to the input image. The subsequent processes are similar to that of GFN, which follows the sequence of GAP, 1x1 convolution, BatchNorm+ReLu, FC, Softmax and cross-entropy loss.

\begin{figure}
\centering
\includegraphics[width=\linewidth]{latex/images/PFN.jpg}
\caption{The PFN divides the feature map X into six horizontal strips and performs peak neuron responses detection to extract the important features within that localized regions. The ROIs are calculated based on those regions and used to crop feature map X for further learning. Best viewed in color.}
\label{fig:PFN}
\end{figure}


\begin{figure}
\centering
\includegraphics[width=\linewidth]{latex/images/attr_classifiers.jpg}
\caption{12 attributes are generated from global, top, middle and bottom vectors on Market1501 dataset.}
\label{fig:attr_classifiers}
\end{figure}

\begin{figure*}
\centering
\includegraphics[scale=0.35]{latex/images/attr_to_aam.jpg}
\caption{On Market1501 dataset, there are a total of 12 attention maps to be used. Eight of the more important attributes are shown above. Only six of those with strong visual cues are selected for AAM merging. ID attention map is obtained from GFN, and is shown here for qualitative comparison with other attributes. Backpack, handbag, bag and hat attributes, though provides good visual cue do not appear in all images, and are therefore dropped. Note that sleeves attention map captures too much background information and thus unsuitable for AAM . Best viewed in color}
\label{fig:attrs_to_aam}
\end{figure*}

\subsection{Attribute classification and AAM}

\par In the AFN, we use Class-Activation Mapping (CAM) \cite{zhou2016learning} as the object detector to localize the regions belonging to the person attributes. Only those attributes which exhibit strong visual cue of the human subject are combined to form a map with strong discriminatory features. This idea is shown in Figure \ref{fig:MergedAttribute}. Since the objective of this task is not semantic segmentation, the AAM does not fully overlap with the human subject. However, we can see from Figure \ref{fig:MergedAttribute} that the produced combined map gives us strong discriminatory features. The spatial location(s) of the attribute object(s), and the spatial relationships among them are well captured. In addition, the attention map helps to remove the background clutter. To demonstrate the effectiveness of AFN, a comparison between of the AAM and the class activation map generated by the global classiﬁcation network, also called the global ID heatmap, are shown in Figure \ref{fig:AAM_Heatmap}. The AAM follows the pedestrian shape more closely, whereas the global ID heat map reveals whatever regions that the trained network thinks are discriminatory for ID classiﬁcation, which explains why ID classiﬁcation alone tends to over-ﬁt. Thus, AAM helps to regularize the main task. 


AFN is the main focus of AANet, and it consists of two sub-tasks. The first sub-task performs classification on individual person attributes. The second sub-task leverage on the output of first sub-task and performs CAM \cite{zhou2016learning} to obtain the class-aware regions. These regions are combined to form a feature map that attempts to resemble that of a person. In this way, the background regions can be removed, and the class related regions, which are very discriminatory features from CAM, can be combined for network learning. The lower half of Figure \ref{fig:AANet} shows the AFN. 
%Figure \ref{fig:AAM_Heatmap} shows the heatmaps of AAM and ID. AAM clearly has more relevant attention regions than the ID feature map, and they reside on the person body region. 

\textbf{Individual attribute classification:} 
The first sub-task of AFN is to perform attributes classification. There are 10 and 12 annotated attributes on DuketMTMC-reID and Market1501 respectively. The first layer of AFN is a 1x1 convolution that downsized the channel depth of feature map X from z to v, which is 2048 to 256. Next we partition the feature maps into three different sets, namely the Top, Middle and Bottom feature maps, each responsible for extracting their localized regions. This is a straight forward way of reducing the background clutters and unwanted signals, boosting the strength of the needed features. For example, the Top feature maps are used for hat, hair, sleeves and upper clothing color attributes features extraction only. Signals from the lower half of the feature maps are effectively removed. As shown in Figure \ref{fig:attr_classifiers}, the outputs of these feature maps are average pooled to become V layers. Together with the output of GFN V layer, which provide the global features, these four set of vectors, with duplication, are fed into their respective fully connected C layers to create 12 sets of attribute representations for Softmax normalization.

\par \textbf{AAM:} This is the task that perform person identity classification on combined map of class sensitive regions from individual attributes, and is shown in Figure \ref{fig:AANet}. The regions are extracted by CAM and merged in AAM before forwarded to AAM classifier. The work flow of this task is shown in Figure \ref{fig:attrs_to_aam}. The first CAM heatmap, denoted as ID, is generated from GFN, and used here as qualitative comparison only. The rest of the attributes CAM heatmaps are obtained from AFN. The feature map input (Top, Middle, Bottom or Global) to the CAM determines the heatmap size and spatial location. The highlighted regions on the heatmaps are the class-sensitive neurons extracted by the CAM. If we refer to the Upper clothing color heatmap on the top row, we can see that the extracted regions corresponds well to the white upper clothing of the query image. Same observations can be made on the rest of Upper clothing color heatmaps, and other attribute heatmaps. 
\par To produce a good AAM, the CAM output has to produce body part well, and available for all images. Out of all the 12 attributes, the gender, hair, upper and lower clothing colors, lower clothing type and length are good choices for AAM merging. The merged AAM is then threshold to remove all unwanted non-class sensitive regions. An example of noise removal is illustrated in the second query, where the Lower clothing color heatmap contains some background clutters, but is effectively removed after AAM thresholding. When comparing to the ID heatmap from GFN, we can see that the final AAM placed different emphasis on the feature maps and thus provides relevant but unique learning experience to the network.

\subsection{Loss calculation}
AANet is a multitask network. The contribution of each task needs to be fine-tuned to obtain optimal accuracy performance. In our work, we utilize homoscedastic uncertainty learning to obtain the task loss weights, and use those weights for person re-ID training. The multitask loss function of the AANet is defined as follows:
\begin{align}
%  L_{global}(y^G,d) & = %-\sum_{i=1}^{C}log(\frac{exp(y_i^G)}{\sum_{c=1}^{C}exp(y_c^G)}q(i)
    \mathcal{L}_{total}(x;\theta;\lambda) = \sum_{i=0}^{T}\lambda_i\mathcal{L}_i(x;\theta)
\end{align}
Where x is a set of training images, \(\theta\)  is the network parameters learned by minimizing \(\mathcal{L}_{total}\). \(T\) is the total number of task loss \(\mathcal{L}_i\). \(\lambda_i\) is the weighting we obtained from uncertainty learning. \(\mathcal{L}_{total}\) is thus given as
%L_total=λ_1 L_global+ λ_2 L_part+ λ_3 L_attribute		    %     (2)
\begin{align}
    \mathcal{L}_{total} = \lambda_g\mathcal{L}_{global} + \lambda_p\mathcal{L}_{part} +
    \lambda_a\mathcal{L}_{attr} + \lambda_{aam}\mathcal{L}_{aam}
\end{align}
Where \(\mathcal{L}_{global}\), \(\mathcal{L}_{part}\), \(\mathcal{L}_{attr}\) and \(\mathcal{L}_{aam}\) are the task losses of GFN, PFN and AFN (attribute and aam) respectively. All task losses are computed as cross-entropy losses during training. When testing for accuracy performance, we concatenate all the outputs of V layers to form a descriptor of 2816 dimensions, for every query and gallery images, and perform \(l_2\) norm to rank them.

\subsection{Implementation}
We implemented AANet with both ResNet-50 and ResNet-152 as backbone network, and pretrained with ImageNet. Images are enlarged to 384 x 128, with only random ﬂip as data augmentation. Batch size is set to 32 for ResNet-50, and 24 for ResNet-152. Using Stochastic Gradient Descent (SGD) as the optimizer, we train the network for 40 epoch. Learning rate starts at 0.1 for the newly added layers, and 0.01 for the pretrained ResNet parameters, and follows the staircase schedule at 20 epoch with a 0.1 reduction factor for all parameters.

\section{Classification Experiments}
\label{sec:results}
In the following experiments, we used the DukeMTMC-reID \cite{ristani2016performance} and Market1501 \cite{DBLP:conf/iccv/ZhengSTWWT15} datasets to conduct our training and testing. DukeMTMC-reID is a subset of DukeMTMC dataset. The images are cropped from videos taken from 8 cameras. The dataset consists of 16,522 training images and 17,661 gallery images, with 702 identities for both training and testing. 408 distractor IDs are also included in the dataset. There are a total of 23 attributes annotated by Lin \etal \cite{DBLP:journals/corr/LinZZWY17}. We use all attributes, but with modification to the clothing color attributes. We merged all 8 upper clothing color attributes and 7 lower clothing color attribute into a single upper clothing attribute and a single lower clothing attribute respectively. 

\par For Market1501, there are a total of 32,668 images for both training and testing. There are 751 identities allocated for training and 750 identities for testing. Lin \etal \cite{DBLP:journals/corr/LinZZWY17} also annotated this dataset, but with 27 person attributes. We use the same clothing color strategy as in DukeMTMC-reID, and use all attributes for training our model.


\subsection{Comparison with the state-of-the-art methods}

\par\textbf{DukeMTMC-reID dataset:} As shown in Table \ref{table:compare_duke}, we have three comparisons. First comparison is on networks trained with smaller backbone model, which in this case is ResNet-50. The three comparison networks are KPM (Res-50) \cite{shen2018end}, PCB (Res-50)\cite{Sun_2018_ECCV} and our AANet-50. We outperformed the best state-of-the-art method \cite{Sun_2018_ECCV} in this category in accuracy by 3.36\% mAP and 3.12\% Rank-1.

\par The second comparison is on networks using larger backbone models, which include both ResNet-101 and ResNet-152. The three comparison networks are GP-reID (Res-101) \cite{almazan2018re}, SPReID (Res-152) \cite{kalayeh2018human} and our AANet-101. Here, we again outperformed the state-of-the-art method \cite{kalayeh2018human} by  1.04\% mAP and 1.79\% Rank-1 accuracy.

\par The third comparison is on networks from second comparison, but this time with Re-Ranking \cite{DBLP:conf/cvpr/ZhongZCL17}. We outperformed the state-of-the-art method \cite{almazan2018re} in accuracy by 2.05\% mAP and 1.52\% Rank-1.

\setlength{\tabcolsep}{8pt}
\begin{table}
\begin{center}
\begin{tabular}{l c c}
\hline\noalign{\smallskip}
\multicolumn{3}{c}{DukeMTMC-reID}\\
Methods & mAP & Rank-1\\
\noalign{\smallskip}
\hline
\noalign{\smallskip}
%LOMO+XQDA \cite{DBLP:conf/cvpr/LiaoHZL15} & 17.0 & 30.8\\
%GAN	\cite{DBLP:conf/iccv/ZhengZY17} & 47.1 & 67.7\\
%APR \cite{DBLP:journals/corr/LinZZWY17} & 51.9 & 70.7\\
%PAN	\cite{DBLP:journals/corr/ZhengZY17aa} & 51.5 & 71.6\\
FMN \cite{DBLP:journals/corr/abs-1711-07155} & 56.9 & 74.5\\
SVDNet \cite{DBLP:conf/iccv/SunZDW17} & 56.8 & 76.7\\
DPFL \cite{DBLP:conf/iccvw/ChenZG17} & 60.6 & 79.2\\
\hline
KPM (Res-50) \cite{shen2018end} & 63.2 & 80.3\\
PCB (Res-50)\cite{Sun_2018_ECCV} & 69.2 & 83.3\\
{\bf Proposed AANet-50}	& {\bf72.56} & {\bf86.42}\\
\hline
GP-reID (Res-101) \cite{almazan2018re} * & 72.80 & 85.20 \\
SPReID (Res-152) \cite{kalayeh2018human} & 73.34 & 85.95 \\ 
{\bf Proposed AANet-152}	& {\bf74.38} & {\bf87.74}\\
\hline
GP-reID (Res-101)\cite{almazan2018re} + RR * & 85.60 & 89.40 \\
SPReID (Res-152)\cite{kalayeh2018human} + RR & 84.99 & 88.96 \\ 
{\bf Proposed AANet-152 + RR} & {\bf87.04} & {\bf90.48}\\
\hline
\end{tabular}
\end{center}
\caption{Performance comparison with other state-of-the-art methods using DukeMTMC-reID dataset. AANet-50 denotes AANet trained using ResNet-50. AANet-101 denotes AANet trained using ResNet-101. RR deonotes Re-Ranking\cite{DBLP:conf/cvpr/ZhongZCL17}
\label{table:compare_duke}. * indicates methods published only in arXiv.}
\end{table}
\setlength{\tabcolsep}{1.4pt}

\par \textbf{Market1501 dataset:} Referring to Table \ref{table:compare_market1501}, we perform similar comparisons as in previous section, but this time using the Market1501 dataset. In the first comparison, which uses ResNet-50, the networks selected are KPM (Res-50) \cite{shen2018end}, PCB (Res-50)\cite{Sun_2018_ECCV} and our AANet-50. We outperformed the best state-of-the-art method \cite{Sun_2018_ECCV} in this category in accuracy by 0.8\% mAP and 0.07\% Rank-1.

\par The second comparison is make using GP-reID (Res-101) \cite{almazan2018re}, SPReID (Res-152) \cite{kalayeh2018human} and our AANet-101, with either ResNet-101 or ResNet152. Here, we again outperformed the state-of-the-art method \cite{kalayeh2018human} in accuracy by 0.05\% mAP and 0.25\% Rank-1.

\par The third Re-Ranking \cite{DBLP:conf/cvpr/ZhongZCL17} comparison is make on networks from second comparison. We outperformed the state-of-the-art method \cite{kalayeh2018human} in accuracy by 1.42\% mAP and 0.47\% Rank-1.

\setlength{\tabcolsep}{1pt}
\begin{table}
\begin{center}
\begin{tabular}{l c c c c}
\hline\noalign{\smallskip}
\multicolumn{5}{c}{Market1501}\\
Methods & mAP & Rank1 & Rank5 & Rank10\\
\noalign{\smallskip}
\hline
\noalign{\smallskip}
%PAR \cite{DBLP:conf/iccv/ZhaoLZW17} & 63.4 & 81.0 & 92.0 & 94.7\\
%MultiLoss \cite{DBLP:conf/ijcai/LiZG17} & 64.4 & 83.9 & - & -\\
%PDC \cite{DBLP:conf/iccv/SuLZX0T17} & 63.4 & 84.4 & 92.7 & 94.9\\
PL-Net \cite{DBLP:journals/corr/YaoZZLT17} & 69.3 & 88.2 & - &	-\\
DPFL \cite{DBLP:conf/iccvw/ChenZG17} & 73.1 & 88.9	& -	& -\\
GLAD \cite{DBLP:conf/mm/WeiZY0T17} & 73.9 & 89.9 & - & -\\
\hline
KPM (Res-50)\cite{shen2018end} & 75.3 & 90.1 & 96.7 & 97.9\\
PCB (Res-50)\cite{Sun_2018_ECCV} & 81.6 & 93.8 & 97.5 & 98.5\\
{\bf Proposed AANet-50} & {\bf82.40} & {\bf93.87} & {\bf97.61} & {\bf98.56}\\
\hline
GP-reID (Res-101) \cite{almazan2018re}* & 81.20 & 92.20 & \bf97.90 & - \\
SPReID (Res-152) \cite{kalayeh2018human} & 83.36 & 93.68 & 97.57 & 98.40 \\ 
{\bf Proposed AANet-152} & {\bf83.41} & {\bf93.93} & {97.64} & {\bf98.53}\\
\hline
GP-reID (Res-101)\cite{almazan2018re}+RR* & 90.00 & 93.00 & 95.90 & - \\
SPReID (Res-152)\cite{kalayeh2018human}+RR & 90.96 & 94.63 & 96.82 & 97.65 \\ 
{\bf Proposed AANet-152+RR} & {\bf92.38} & {\bf95.10} & {\bf97.32} & {\bf97.94}\\
\hline
\end{tabular}
\end{center}
\caption{Performance comparison with other state-of-the-art methods using Market1501 dataset. AANet-50 denotes AANet trained using ResNet-50. AANet-152 denotes AANet trained using ResNet-152. RR denotes  Re-Ranking\cite{DBLP:conf/cvpr/ZhongZCL17}. * indicates methods published only in arXiv.
 }
\label{table:compare_market1501}
\end{table}
\setlength{\tabcolsep}{1.4pt}

\subsection{Further analysis and comparisons}
We now take a closer look at some of the results obtained from our ablation study, the impact of input image resolution and the size of the backbone network. We will also review the design strategies that affects the attribute attention map.

\par \textbf{Ablation study:} In Table \ref{table:duke_ablation_study}, we shows the ablation study on the impact of the task loss weights on AANet accuracy performance using DukeMTMC-reID dataset. The ID task, the part task, the attribute task and the attribute attention task are denoted as \(\mathcal{L}_g\), \(\mathcal{L}_p\), \(\mathcal{L}_a\) and \(\mathcal{L}_{aa}\) respectively. 
As we add each of these relevant tasks to the network, the accuracy improves, which is what we have expected for multitask network. When we use homoscedastic uncertainty learning to obtain the task loss weights \(\mathcal{L}_g\), \(\mathcal{L}_p\) and \(\mathcal{L}_a\), the accuracy improves to 70.47\% mAP and 85.44\% Rank-1. This result alone is enough to outperform the best state-of-the-art method using ResNet50. With the integration of AAM to the AFN, we push the accuracy result up to 72.56\% mAP and 86.42\%. This strongly indicates that network performance can be enhanced by discovering the features hidden within the CNN layers.

\par \textbf{Comparison of backbone networks:} As shown by Kalayeh \etal \cite{kalayeh2018human} and Almazan \etal \cite{almazan2018re}, the depth of the backbone network affects the accuracy performance of person re-ID. Deeper networks yields better result, and this is clearly shown in both Table \ref{table:compare_duke} and \ref{table:compare_market1501}. In fact, this applies to other computer vision task, like image segmentation, too. However, it gets more expensive, in terms of memory consumption and training time, as we add more layers to the model. If we take a closer look at Table \ref{table:compare_duke}, our AANet-50's Rank-1 accuracy outperformed SPReID (Res-152)'s \cite{kalayeh2018human} Rank-1 accuracy by 0.47\%, and GP-reID (Res-101)'s \cite{almazan2018re} Rank-1 accuracy by 1.22\%. We achieved similar Rank-1 result on Market1501 dataset also, with our AANet-50 outperforming those using deeper backbone networks. This shows the important of diligently searching for features hidden within the CNN, especially when there are relevant but unique tasks added to assist the main objective. 

\par \textbf{Comparison of training processes:} \cite{kalayeh2018human} and \cite{almazan2018re} use rather elaborate methods to enhance their accuracy performance. \cite{kalayeh2018human} aggregates a total of 10 different datasets to generate $\sim$ 111k images and $\sim$ 17k identities for training and testing their network. In addition, they have a fine-tuning process where they initially train their network fully with image size of 492x164, and later fine-tune it with images enlarged to 748x246. \cite{almazan2018re} on the other hand requires practices such as pre-training for identity classification before regression learning, large image size, hard triplet mining and deeper backbone network. Our AANet uses smaller image size, need just a single dataset for each benchmark, simpler training process, and a less shallow ResNet-50 to rival both works.
%mention about X dimension, number of parts
%Thresholding for both part and attribute

\setlength{\tabcolsep}{4pt}
\begin{table}
\begin{center}
\begin{tabular}{ | l | C{0.3cm} | C{0.3cm} | C{0.3cm} | C{0.3cm} | C{0.85cm} | C{0.85cm} |}
\hline%\noalign{\smallskip}
%\multicolumn{1}{l|}{} & \multicolumn{3}{c|}{} & %\multicolumn{2}{c|}{Classification} & \multicolumn{1}{c}{}\\
%\multicolumn{1}{|l|}{} & \multicolumn{3}{c|}{} & \multicolumn{2}{c|}{Accuracy}\\
%\cline{5-6}
\multicolumn{1}{|l|}{AANet-50} & \multicolumn{4}{c|}{Task} & \multicolumn{1}{c|}{mAP} & \multicolumn{1}{c|}{Rank 1}\\
\multicolumn{1}{|l|}{Task Loss} & \multicolumn{4}{c|}{Weights} & \multicolumn{1}{c|}{\%} & \multicolumn{1}{c|}{\%}\\
\hline
\(\mathcal{L}_g\) & 1 & 0 & 0 & 0 & 62.92 & 80.18\\
%\(\mathcal{L}_p\) & 0 & 1 & 0 & 74.3 & 91.0\\
%\(\mathcal{L}_a\) & 0 & 0 & 1 & - & -\\
%\(\mathcal{L}_g + \mathcal{L}_a\) & 1 & 0 & 1 & 75.5 & 90.3\\
\(\mathcal{L}_g + \mathcal{L}_p\) & 1 & 1 & 0 & 0 & 66.35 & 82.93\\
\(\mathcal{L}_g + \mathcal{L}_p + \mathcal{L}_a\) & 1 & 1 & 1 & 0 & 67.28 & 83.29\\
\hline
\multicolumn{1}{|l|}{\(\mathcal{L}_g + \mathcal{L}_p\ + \mathcal{L}_a\)} & \multicolumn{4}{c|}{Uncertainty} & \multicolumn{1}{c|}{70.47} & \multicolumn{1}{c|}{85.44}\\
\multicolumn{1}{|l|}{\(\mathcal{L}_g + \mathcal{L}_p + \mathcal{L}_a + \mathcal{L}_{aa}\)} & \multicolumn{4}{c|}{Learning} & \multicolumn{1}{c|}{\textbf{72.56}} & \multicolumn{1}{c|}{\textbf{86.42}}\\
\hline
\end{tabular}
\end{center}
\caption{Performance comparisons of different combination of task losses using DukeMTMC-reID dataset, with and without uncertainty learning. The top three rows are AANet accuracy with equal weights to the tasks. Bottom two rows show the results with loss weights obtained from uncertainty learning.
}
\label{table:duke_ablation_study}
\end{table}
\setlength{\tabcolsep}{1.4pt}

\begin{figure}
\centering
\includegraphics[width=\linewidth]{latex/images/Image_retrieval_good.jpg}
\caption{Three good queries from the DukeMTMC-reID with eight retrieved images for each query.}
\label{fig:good_retrieval}
\end{figure}


\begin{figure*}
\centering
\includegraphics[width=\linewidth]{latex/images/attr_query.jpg}
\caption{Three examples of how person attributes help in improving the image retrieval accuracy. First row used gender and color attributes to filter the retrieved images to get correct images within the top 5 ranks. Second row used hat, color and gender attributes to achieve same result as first row. Last row used color and backpack attributes to filter away falsely accepted images. Green box denotes same ID as query image. Red box denotes different ID from query image. Best viewed in color}
\label{fig:attr_query}
\end{figure*}

\setlength{\tabcolsep}{4pt}
\begin{table*}
\begin{center}
\begin{tabular}{ l | c c c c c c c c c c c c | c }
\hline
Methods & gender & age & hair & L.slv & L.low & S.clth & B.pack & H.bag & bag & hat & C.up & C.low & mean\\
\hline
APR \cite{DBLP:journals/corr/LinZZWY17} & 86.45 & 87.08 & 83.65 & 93.66 & 93.32 & 91.46 & 82.79 & 88.98 & 75.07 & 97.13 & 73.40 & 69.91 & 85.33\\
AANet-152 & {\bf92.31} & {\bf88.21} & {\bf86.58} & {\bf94.45} & {\bf94.24} & {\bf94.83} & {\bf87.77} & {\bf89.61} & {\bf79.72} & {\bf98.01} & {\bf77.08} & {\bf70.81} & {\bf87.80}\\
\hline
\end{tabular}
\end{center}
\caption{Performance comparisons of attribute accuracy on Market1501 dataset.
}
\label{table:attr_accuracy}
\end{table*}
\setlength{\tabcolsep}{1.4pt}

\section{Attribute Experiments}
In this section, we illustrate how person attributes help in refining the retrieved images for image-based identity classification task. We also show the accuracy of person attributes.

\subsection{Retrieval results}
As shown in Figure \ref{fig:good_retrieval}, we have three examples of good image retrievals from AANet. Though there are some occlusions on the query subjects, for examples, tree, cars and unwanted pedestrian, AANet has no problem retrieving correct images from the gallery set.
\par Next, we show some examples of challenging queries, where the subjects are heavily occluded, and resulted in poor retrieval accuracy. We demonstrate how person attributes help to filter out the incorrect retrievals. This is shown in \ref{fig:attr_query}. Three examples are given, each with their own retrieval difficulties. First example is given in row one. More than half of the query subject was not visible, and the upper clothing color was similar to the other pedestrian clothing. Out of the top 10 images retrieved, only one correct identity was found. To filter away the wrong identities, we use person attribute query, by specifying male and white lower clothing color attributes as search criteria, and compare them with the predicted attributes of the retrieved images. AANet successfully returns correct identity images within the top 5 ranks. For row two, we have similar challenging query. The query subject is the lady in green and red clothing, but the retrieved images point to identities wearing white clothing only as that matches more closely to the query image. The correct images actually ranked from 14 to 21. To get the right images, we specified green and red clothing color attributes, gender attribute and hat attribute to effectively remove all those false retrievals, leaving us the images from correct identity. In last row, we are given another difficult retrieval task. The subject is severely occluded, and has very similar attributes as found in those incorrect retrievals. We relied on black and gray clothing colors, and backpack attributes to retrieve all correct images within the top 5 rank.

\subsection{Attribute accuracy performance}
The attribute accuracy performance comparison between AANet and APR \cite{DBLP:journals/corr/LinZZWY17} is shown in Table \ref{table:attr_accuracy}. APR \cite{DBLP:journals/corr/LinZZWY17} is provided by Lin \etal, the author who annotated the DukeMTMC-reID and Market1501 datasets with person attributes. As shown, AANet outperforms APR on all attributes. %It is worth noting that color related attributes, like the upper and lower clothing colors, do not perform well for both networks when compared to the rest of the attributes. The reason being cameras used to take videos or images are not color calibrated after installation. 
%Nonetheless, it is still very handy when performing image retrieval. 

%\setlength{\tabcolsep}{8pt}
%\begin{table}
%\begin{center}
%\begin{tabular}{l c c}
%\hline\noalign{\smallskip}
%\multicolumn{3}{c}{ResNet-50 AAM Design Parameters}\\
%Methods & mAP & Rank-1\\
%\noalign{\smallskip}
%\hline
%\noalign{\smallskip}
%\hline
%1 vector + no threshold  & 81.99 & 93.50 \\
%1 vector + threshold & 82.04 & 93.48 \\ 
%\hline
%4 vectors + no threshold  & 81.89 & 93.42 \\
%4 vectors + threshold & {\bf82.40} & {\bf93.87} \\
%\hline
%\end{tabular}
%\end{center}
%\caption{Performance comparison on AAM design parameters.}
%\label{table:aam_design_para}
%\end{table}
%\setlength{\tabcolsep}{1.4pt}

%\subsection{ResNet-50 AAM design parameters}
%We tested two crucial AAM parameters to validate our design assumptions. The first is the number of vectors used to generate the attributes. We tested single global vector vs the 4 global, top, middle and bottom vectors. We also tested the effectiveness of thresholding the AAM. The results are shown in Table \ref{table:aam_design_para}, which confirms that global and localized region vectors, and thresholding AAM give the best result. These parameters, in reality, reduce unwanted noise from our intended features, thus allowing our AANet to learn better.



\section{Conclusions}
\label{sec:conclu}
%We showed that our AANet, with the attribute attention map capturing the class sensitive regions, and attenuating the backgrounds, is able to share its unique learning experience with the global identity task, and compliment each others to bring out the very discriminatory features useful for person re-ID task. As a result, we outperformed the best state-of-of-art methods, regardless of the backbone architecture employed. On top of that, our AANet achieves good accuracy on person attribute prediction. This provides our user a very efficient and flexible image retrieval system.
%\par One area which we think we can pursue in the future is to leverage on those under utilized attributes to create a more complete person attention map.
In this paper we proposed a novel architecture to incorporate attributes based on physical appearance such as clothing color, hair, presence/absence of backpack etc. into a classification based person re-id framework. The propsosed Attribute Attenion Network (AANet) employs joint end-to-end learning and uncertainty learning for multitask loss fusion. The resulting network outperforms existing state-of-the-art re-id solutions on multiple benchmark datasets. In addition, AANet produces textual descriptions of the queried image based on the queried person’s physical attributes. This enables text-based query in addition to the traditional image-based query for re-ID. The AANet, to the best of our knowledge, is the first unified framework that allows both image and text-based queries for person re-ID.
{\small
\bibliographystyle{ieee}
\bibliography{egbib}
}
%\end{multicols}
\end{document}

